Finite-time transitions in optimal control and non-equilibrium relaxation

We theoretically and experimentally study finite-time optimal control of a colloidal particle steered through a spatially inhomogeneous environment, modeled by a position-dependent energetic cost at the final state. The competition between this state-dependent penalty and path-dependent dissipation gives rise to a sharp transition in the control strategy at a critical control duration. We further show that this transition can be linked to a dynamical phase transition in nonequilibrium relaxation after a quench, where the control cost maps onto the rate function governing rare trajectories.

==> main-xr.tex <==
\newlabel{M-FirstPage}{{}{1}{}{section*.1}{}}
\newlabel{M-fig:sketch}{{1}{1}{A particle (blue) is driven by a harmonic trap (red) at constant mean horizontal velocity $v_\parallel $ toward an obstacle (green), characterized by an energetic cost $V(x)$. The trap controls the lateral velocity $v_\perp $ to minimize the total work performed on the particle}{figure.1}{}}
\newlabel{M-eq:Langevinequ}{{1}{2}{}{equation.0.1}{}}
\newlabel{M-eq:cost}{{2}{2}{}{equation.0.2}{}}
\newlabel{M-eq:cc3}{{3}{2}{}{equation.0.3}{}}
\newlabel{M-eq:Cmin}{{4}{2}{}{equation.0.4}{}}
\newlabel{M-eq:ddW}{{5}{2}{}{equation.0.5}{}}
\newlabel{M-eq:tcrit}{{6}{2}{}{equation.0.6}{}}
\newlabel{M-eq:lamsol}{{7}{2}{}{equation.0.7}{}}
\newlabel{M-eq:Upot}{{8}{3}{}{equation.0.8}{}}
\newlabel{M-eq:Vx}{{9}{3}{}{equation.0.9}{}}
\newlabel{M-fig:protocols}{{2}{3}{Optimal control protocols for different average initial positions $u_0$ (dashed) and experimental trajectories [solid red in (a), blue in (b)], with process durations: (a) $t_f=0.47\,t_\text {c}$, and (b) $t_f=1.65\,t_\text {c}$. (c) $\ms {W}_{t_f}^*$ at $u_0=0$ as a function of $t_f$ from experiments (markers) and theory (line) for $V_0 = \kappa x_\text {m}^2 = 151\,\kb T$ (d) $\ms {W}_{t_f}^*$ as a function of $u_0$ at $t_f = 0.45\,t_\text {c}$ (red) and $t_f = 1.65\,t_\text {c}$ (blue). Results from experiments (markers) and theory (lines) for $V_0 = \kappa x_\text {m}^2 = 124\,\kb T$. $\tilde V(u_f)$ is shown in green. Inset: $|u^*_f|$ as a function of the control time $t_f$ (yellow) from experiments (markers) and theory (solid line)}{figure.2}{}}
\newlabel{M-eq:V0t}{{10}{4}{}{equation.0.10}{}}
\newlabel{M-fig:ratefunc_relax}{{3}{4}{Results of the free-relaxation experiment, post-processed with the reweighting method, for $V_0 = 40\,\kb T$ from $2\cdot 10^3$ trajectories. (a) Rate function $\ms {V}^*_{t_f}$ as a function of $x_f$, for different $t_f$. (b) Order parameter density $P(|x_0|,t_f)$ as a function of $t_f$ from experiments (heat map) and $|x^*_0|$ from theory (solid line). $P(|x_0|,t_f)$ is scaled to unity at each $t_f$ to improve visibility. (c) Trajectory density of relaxation trajectories that reach $x_f=0$ at different times $t_f$ from experiment (heat map), combined for $t_f=0.55t^R_\text {c}$ and $t=2t^R_\text {c}$. Solid lines show the theoretical predictions. (d) Susceptibility of the order parameter $x_0$ as a function $t_f$ at $V_0=10\,\kb T$, $20\,\kb T$, $30\,\kb T$, and $40\,\kb T$ (from light to dark). Inset: Scaling behavior of $\chi _t$}{figure.3}{}}
\newlabel{M-LastBibItem}{{33}{6}{}{section*.11}{}}
\newlabel{M-LastPage}{{}{6}{}{}{}}

